Optimizing Batch Linear Queries under Exact and Approximate Differential Privacy

Differential privacy is a promising privacy-preserving paradigm for statistical query processing over sensitive data. It works by injecting random noise into each query result, such that it is provably hard for the adversary to infer the presence or absence of any individual record from the published noisy results. The main objective in differentially private query processing is to maximize the accuracy of the query results, while satisfying the privacy guarantees. Previous work, notably \cite{LHR+10}, has suggested that with an appropriate strategy, processing a batch of correlated queries as a whole achieves considerably higher accuracy than answering them individually. However, to our knowledge there is currently no practical solution to find such a strategy for an arbitrary query batch; existing methods either return strategies of poor quality (often worse than naive methods) or require prohibitively expensive computations for even moderately large domains. Motivated by this, we propose low-rank mechanism (LRM), the first practical differentially private technique for answering batch linear queries with high accuracy. LRM works for both exact (i.e., $\epsilon$-) and approximate (i.e., ($\epsilon$, $\delta$)-) differential privacy definitions. We derive the utility guarantees of LRM, and provide guidance on how to set the privacy parameters given the user's utility expectation. Extensive experiments using real data demonstrate that our proposed method consistently outperforms state-of-the-art query processing solutions under differential privacy, by large margins.

==> abs.tex <==
%Differential privacy is a promising privacy-preserving paradigm for
%statistical query processing over sensitive data. It works by
%injecting random noise into each query result, such that it is
%provably hard for the adversary to infer the presence or absence of
%any individual record from the published noisy results. The main
%objective in differentially private query processing is to maximize
%the accuracy of the query results, while satisfying the privacy
%guarantees. Previous work, notably the matrix mechanism
%\cite{LHR+10}, has suggested that processing a batch of correlated
%queries as a whole can potentially achieve considerable accuracy
%gains, compared to answering them individually. However, as we point
%out in this paper, the matrix mechanism is mainly of theoretical
%interest; in particular, several inherent problems in its design
%limit its accuracy in practice, which almost never exceeds that of
%na\"{\i}ve methods. In fact, we are not aware of any existing
%solution that can effectively optimize a query batch under
%differential privacy. Motivated by this, we propose the
%\emph{Low-Rank Mechanism} (LRM), the first practical differentially
%private technique for answering batch queries with high accuracy,
%based on a \emph{low rank approximation} of the workload matrix. We
%prove that the accuracy provided by LRM is close to the theoretical
%lower bound for any mechanism to answer a batch of queries under
%differential privacy. Extensive experiments using real data
%demonstrate that LRM consistently outperforms state-of-the-art query
%processing solutions under differential privacy, by large margins.


Differential privacy is a promising privacy-preserving paradigm for
statistical query processing over sensitive data. It works by
injecting random noise into each query result, such that it is
provably hard for the adversary to infer the presence or absence of
any individual record from the published noisy results. The main
objective in differentially private query processing is to maximize
the accuracy of the query results, while satisfying the privacy
guarantees. Previous work, notably \cite{LHR+10}, has suggested that with an appropriate strategy, processing a batch of correlated
queries as a whole achieves considerably higher accuracy
than answering them individually. However, to our knowledge there is currently no practical solution to find such a strategy for an arbitrary query batch; existing methods either return strategies of poor quality (often worse than naive methods) or require prohibitively expensive computations for even moderately large domains. Motivated by this, we propose the \emph{Low-Rank Mechanism} (LRM), the first practical
differentially private technique for answering batch queries with
high accuracy, based on a \emph{low rank approximation} of the
workload matrix. We prove that the accuracy provided by LRM is close
to the theoretical lower bound for any mechanism to answer a batch
of queries under differential privacy. Extensive experiments using
real data demonstrate that LRM consistently outperforms
state-of-the-art query processing solutions under differential
privacy, by large margins.


==> dat.tex <==
\section{Constrained Inference in Low-Rank Mechanism}
Our low-rank mechanism is a data-independent method, it is not possible to optimize for relative error directly. However,if the prior information of the target dataset were known, we could use some constrained inference techniques to improve the accuracy of the basic algorithm of our low-rank mechanism. 

\cite{HRMS10,hay2009accurate} introduce a post-processing technique that operates on the output of Algorithm 1.
\cite{LZMY11} compresses the data 

We make the following assumptions.
(i) Bound assumption. We assume 

A variety of data relate to quantities representing physical constants are nonnegative values. So we assume the data only contains nonnegative entries. (ii) Non-increasing Data.

(iii) Large Range and Sparse Data.

 

The main idea behind the approach is to use the semantics of a query to impose constraints on the answer. While the true answer always satisfies the constraints, the noisy answer that is output by the low-rank mechanism may violet them. Let $y$ denote the im

output of low-rank mechanism, the constrained inference process takes $y$ and find the answer that is close to $y$ while also satisfies the constraints of the query. Here closest is measured in $_2$ distance. The algorithm is summarized in Algorithm 4
.

As discussed in , the technique has no impact on privacy since it requires no access to the private databases, only $y$ the output of the differentially private algorithms.


nonnegative data, 



\begin{algorithm}[t]
\caption{\label{algorithm:data_aware_opt} {\bf Constrained Inference in Low-Rank Mechanism}}
\begin{algorithmic}[1]
  \STATE input: workload matrix $W\in R^{m \times n}$, data vector $x \in R^{n \times 1}$, $C$ and $k$
  \STATE Solve the workload matrix decomposition problem:
  \begin{center}
  \begin{tabular}{c}
    $\min_{B,L}~~ \frac{1}{2}tr(B^TB)$       \\
    $s.t. ~~ W=BL, ~~ \forall j \sum_i^r |L_{ij}|\leq 1$      \\
  \end{tabular}
  \end{center}
  \STATE Draw a noise vector $b\in R^{r \times 1}$ from the corresponding Laplacian distribution or Gaussian distribution
  \STATE Compute $y$: $y = Lx + b$
  \STATE Solve the following optimization problems:
  \begin{center}
  \begin{tabular}{c}
    $\min_v  \|y - L v\|_2^2$       \\
    $s.t. ~~ \|v\|_0 \leq k$        \\
    $v_1  \leq  v_2  \leq ... \leq v_n$      \\
    $  v_1 \leq  C, ~~ v_n \geq 0 $     \\
  \end{tabular}
  \end{center}
  \STATE output: BLv
\end{algorithmic}
\end{algorithm}




